HexPlane: A Fast Representation for Dynamic Scenes

Modeling and re-rendering dynamic 3D scenes is a challenging task in 3D vision. Prior approaches build on NeRF and rely on implicit representations. This is slow since it requires many MLP evaluations, constraining real-world applications. We show that dynamic 3D scenes can be explicitly represented by six planes of learned features, leading to an elegant solution we call HexPlane. A HexPlane computes features for points in spacetime by fusing vectors extracted from each plane, which is highly efficient. Pairing a HexPlane with a tiny MLP to regress output colors and training via volume rendering gives impressive results for novel view synthesis on dynamic scenes, matching the image quality of prior work but reducing training time by more than $100\times$. Extensive ablations confirm our HexPlane design and show that it is robust to different feature fusion mechanisms, coordinate systems, and decoding mechanisms. HexPlane is a simple and effective solution for representing 4D volumes, and we hope they can broadly contribute to modeling spacetime for dynamic 3D scenes.

==> figures/fusion_aba.tex <==

\begin{figure}[!htp]
    \centering
    \resizebox{0.48\textwidth}{!}{
    \begin{tabular}{@{}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{}}
    % \includegraphics[width=0.24\textwidth]{./figures/material/synth_results/flame_salmon_21.png}&
    % \includegraphics[width=0.24\textwidth]{./figures/material/synth_results/flame_salmon_38.png}&
    % \includegraphics[width=0.24\textwidth]{./figures/material/synth_results/flame_salmon_54.png}&
    % \includegraphics[width=0.24\textwidth]{./figures/material/synth_results/flame_salmon_76.png}\\
    \includegraphics[width=0.09\textwidth]{./figures/material/fusion_ablation/images/13_gt.png} &
    \includegraphics[width=0.09\textwidth]{./figures/material/fusion_ablation/images/Prodcut_Concat_13.png} &
    \includegraphics[width=0.09\textwidth]{./figures/material/fusion_ablation/images/Product_SUM_13.png} &
    \includegraphics[width=0.09\textwidth]{./figures/material/fusion_ablation/images/Sum_Product_13.png} &
    \includegraphics[width=0.09\textwidth]{./figures/material/fusion_ablation/images/Sum_Sum_13.png}\\
    \scriptsize{GT} &\scriptsize{Multiply-Concat} & \scriptsize{Multiply-Sum} & \scriptsize{Sum-Multiply} & \scriptsize{Sum-Sum} \\
    \end{tabular}}
    \vspace{-2mm}
    \captionof{figure}{
    \textbf{Synthesis Results with Various Fusion Designs.}
    HexPlane could give reasonable results with different fusion designs.}
    \label{fig:fusion_aba}
    \vspace{-4mm}
    \end{figure}

==> tables/Grid_ablation.tex <==
% \begin{table}[t!]
%     \centering
%     \caption{
%     \textbf{Ablations on different Grid Resolution.}}
%     \vspace{1mm}
%     \resizebox{0.98\textwidth}{!}{
%     \begin{tabular}{ p{2cm} p{2cm} p{3cm} p{3cm} p{3cm}}
%     \toprule[2pt]
%     Rank &Time Grid & $128^3$ &$256^3$  &$512^3$ \\
%     \midrule
%     \multirow{4}{*}{48} & 16\\
%         & 32\\
%         & 128\\
%         & 256\\
%     \midrule   
%     \multirow{4}{*}{96} & 16\\
%         & 32\\
%         & 128\\
%         & 256\\
%     \midrule   
%     \multirow{4}{*}{192} & 16\\
%         & 32\\
%         & 128\\
%         & 256\\
%     % No Position Encoding &  & & &\\
%     \bottomrule [2 pt]
%     \end{tabular}}
%     \label{tab:grid_abalation}
% \end{table}
\begin{table}[t!]
        \centering
        \caption{
        \textbf{Ablations on different Grid Resolution.}}
        \vspace{1mm}
        \resizebox{0.48\textwidth}{!}{
        \begin{tabular}{  p{2cm} p{3cm} p{3cm} p{3cm}}
        \toprule[2pt]
        Time Grid & $128^3$ &$256^3$  &$512^3$ \\
        \midrule
        0.5 & 27.828/0.866/0.198 & 28.702/0.899/0.124 & 28.374/0.909/0.098 \\
        1.0 & 27.960/0.868/0.192 & 28.241/0.899/0.124 & 29.043/0.909/0.096\\
        1.5 & 25.494/0.861/0.203 & 28.819/0.899/0.124 & 28.808/0.910/0.094 \\

        \bottomrule [2 pt]
        \end{tabular}}
        \label{tab:grid_abalation}
    \end{table}
    
